DSLR: Document Refinement with Sentence-Level Re-ranking and Reconstruction to Enhance Retrieval-Augmented Generation

Recent advancements in Large Language Models (LLMs) have significantly improved their performance across various Natural Language Processing (NLP) tasks. However, LLMs still struggle with generating non-factual responses due to limitations in their parametric memory. Retrieval-Augmented Generation (RAG) systems address this issue by incorporating external knowledge with a retrieval module. Despite their successes, however, current RAG systems face challenges with retrieval failures and the limited ability of LLMs to filter out irrelevant information. Therefore, in this work, we propose DSLR (Document Refinement with Sentence-Level Re-ranking and Reconstruction), an unsupervised framework that decomposes retrieved documents into sentences, filters out irrelevant sentences, and reconstructs them again into coherent passages. We experimentally validate DSLR on multiple open-domain QA datasets and the results demonstrate that DSLR significantly enhances the RAG performance over conventional fixed-size passage. Furthermore, our DSLR enhances performance in specific, yet realistic scenarios without the need for additional training, providing an effective and efficient solution for refining retrieved documents in RAG systems.

==> fig/motivation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/model_comparison.pdf}
    \caption{
    Distribution of relevance scores for 1000 randomly sampled documents from the NQ, TQA, and SQD datasets for each model.
    }
    \label{fig:model_comparison}
\end{figure}

==> fig/precision.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/precision.pdf}
    %\caption{Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and passage-level across various open-domain QA datasets.}
    \caption{\small Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and the passage-level baseline (Passage).}
% Comparison of passage-level and sentence-level reranking accuracy (acc) on the NQ dataset. The left graph shows accuracy improvements with increasing context length (\(L\)), and the right graph shows accuracy improvements with increasing initial retrieval depth (\(N\)).}
    \label{fig:precision}
    \vspace{-0.15in}
\end{figure}


==> fig/robustness.tex <==
\begin{figure}[t!]
    \vspace{-0.07in}
    \centering
    \includegraphics[width=1\linewidth]{fig/reranking_strategies_comparison_combined.pdf}
    \caption{\small Comparison of the passage-level baseline and \textit{DSLR} with sentence-level re-ranking by varying context lengths (\(L\)) and initial retrieval depths (\(N\)) on the NQ dataset. %The left graph shows accuracy across varying context lengths (\(L\)), and the right graph details accuracy across different initial retrieval depths (\(N\)).
    }
    \label{fig:robustness}
    \vspace{-0.15in}
\end{figure}

==> table/dense.tex <==

% \begin{table}
%     \centering
%     \small
%     \begin{tabular}{ccccccc}
%  & & & \multicolumn{2}{c}{TOP-20}& \multicolumn{2}{c}{TOP-100}\\
%          \multicolumn{2}{c}{Re-ranker}&  Granularity&  L=100&L=500&L=100&L=500\\
%          \multicolumn{7}{c}{w/o Re-ranking} \\
%  \multicolumn{2}{c}{- }& -& 57.3&64.3&57.3&64.3\\
%  \multicolumn{7}{c}{w Re-ranking} \\
%          \multicolumn{2}{c}{BM25}&  Passage&  57.3&65.4&  53.7&64.2\\
%          \multicolumn{2}{c}{}&  Sentence&  59.5&66.4&  57.3&66.3\\
%          \multicolumn{2}{c}{Contriever}&  Passage&  57.2&64.3&  57.2&64.3\\
%          \multicolumn{2}{c}{}&  Sentence&  59.6&66.4&  59.8&67.4\\
%          \multicolumn{2}{c}{DPR}&  Sentence&  60.5&64.3&  61.2&67.3\\
%          \multicolumn{2}{c}{MonoT5}&  Passage&  64.9&67.8&  66.5&70.9\\
%  \multicolumn{2}{c}{}& Sentence& 65.0&67.9& 67.0&70.4\\
%  \multicolumn{2}{c}{RankT5}& Passage& 64.4&67.7& 65.7&70.2\\
%  \multicolumn{2}{c}{}& Sentence& 64.1&67.7& 66.1&70.2\\
%  \multicolumn{2}{c}{RG}& Passage& 65.3&68.5& 66.4&71.1\\
%  \multicolumn{2}{c}{}& Sentence& 65.4&68.2& 66.9&70.5\\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:dense}
% \end{table}
\begin{table}[t!]
    \centering
    \small
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{ccccccc}
        \toprule
         & & & \multicolumn{2}{c}{\textit{Top-20}} & \multicolumn{2}{c}{\textit{Top-100}} \\
         \cmidrule(lr){4-5} \cmidrule(lr){6-7}
         \multicolumn{2}{c}{Re-ranker} & Granularity & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 \\
         \midrule
         \multicolumn{7}{c}{\textit{w/o Re-ranking}} \\
         \midrule
         \multicolumn{2}{c}{-} & - & 57.3 & 64.3 & 57.3 & 64.3 \\
         \midrule
         \multicolumn{7}{c}{\textit{w Re-ranking}} \\
         \midrule
         \multicolumn{2}{c}{DPR} & Sentence & 60.5 & 64.3 & 61.2 & 67.3 \\
         
         
         \midrule
         \multicolumn{2}{c}{BM25} & Passage & 57.3 & 65.4 & 53.7 & 64.2 \\
         \multicolumn{2}{c}{} & Sentence & 59.5 & 66.4 & 57.3 & 66.3 \\
         \midrule
         
         \multicolumn{2}{c}{Contriever} & Passage & 57.2 & 64.3 & 57.2 & 64.3 \\
         \multicolumn{2}{c}{} & Sentence & 59.6 & 66.4 & 59.8 & 67.4 \\
         \midrule
         \multicolumn{2}{c}{MonoT5} & Passage & 64.9 & 67.8 & 66.5 & 70.9 \\
         \multicolumn{2}{c}{} & Sentence & 65.0 & 67.9 & 67.0 & 70.4 \\
         \midrule
         \multicolumn{2}{c}{RankT5} & Passage & 64.4 & 67.7 & 65.7 & 70.2 \\
         \multicolumn{2}{c}{} & Sentence & 64.1 & 67.7 & 66.1 & 70.2 \\
         \midrule
         \multicolumn{2}{c}{RG} & Passage & 65.3 & 68.5 & 66.4 & 71.1 \\
         \multicolumn{2}{c}{} & Sentence & 65.4 & 68.2 & 66.9 & 70.5 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of different re-ranking methods with dense retrieval (DPR) on the TQA dataset, evaluated at two length levels (\(L\)=100 and \(L\)=500) for Top-20 and Top-100 retrieved documents.}
    \label{tab:dense}
\end{table}


==> table/main1-2.tex <==

\begin{table}
    \centering
    \small
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{c |cc | cc}
    \toprule
         &  \multicolumn{2}{c |}{\textit{Top-20}}&  \multicolumn{2}{c}{\textit{Top-100}}\\
         &  Passage &  Sentence &  Passage& Sentence\\ \midrule
         \textbf{NQ}&  45.5&  48.7&  48.7& 53.2\\
         \textbf{TQA}&  64.4&  67.8&  65.3& 69.3\\
         \textbf{SQD}&  46.2&  53.1&  46.1& 56.0\\
         \textbf{RQA}&  35.0&  44.0&  35.0& 44.0\\
         \textbf{SQ}&  48.4&  53.7&  50.0& 57.3\\
         \textbf{BASQ}&  28.4&  30.9&  26.8& 30.8\\ \midrule
    \textbf{AVG.} & 44.6 & \textbf{49.7} & 45.3 & \textbf{51.8} \\
    \bottomrule
    \end{tabular}
}
    \caption{Average passage precision after reranking for top-20 and top-100 retrieved documents, comparing sentence-level (\(DSLR\)) and passage-level across various open-domain QA datasets.}
    \label{tab:main1-2}
\end{table}

==> table/main1-20.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{lscape}

\begin{table*}[t!]
\caption{\small Comparative performance of sentence-level (\textit{DSLR}) and passage-level re-ranking methods across multiple open-domain QA datasets. Results are presented for two context lengths (\(L\)=100 and \(L\)=500), using sparse and dense retrievers, and both supervised and unsupervised re-rankers, for the top-20 retrieved documents. The best performances are in \textbf{bold}.}
\small
\centering

\begin{threeparttable}
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll | cc | cc | cc | cc | cc | cc | cc}
\toprule 
\multirow{2}{*}{\textbf{Type}}    & \multirow{2}{*}{\textbf{Re-ranker}}             & \multirow{2}{*}{\textbf{Granularity}} & \multicolumn{2}{c|}{\textbf{NQ}}            & \multicolumn{2}{c|}{\textbf{TQA}}           & \multicolumn{2}{c|}{\textbf{SQD}}           & \multicolumn{2}{c|}{\textbf{RQA}\tnote{*}}           & \multicolumn{2}{c|}{\textbf{SQ}} & \multicolumn{2}{c|}{\textbf{BASQ}} & \multicolumn{2}{c}{\textbf{AVG.}}            \\ 

                              &                                    &    & # tok & acc & # tok & acc & # tok & acc & # tok & acc & # tok & acc & # tok & acc & # tok & acc \\ \midrule
\multicolumn{17}{c}{\textit{w/o Re-ranking}}   \\  \midrule
- & - & -  & 25.5  & {34.9}  & 58    & {64.6}  & 28.5  & {35.9}  & 37    & {40.1}  & 33.9  & {40.9}  & 56.8  & {59.5} & 40.0 & 46.0 \\ \midrule
% \multicolumn{17}{c}{\textit{w/Re-ranking}}   \\  \midrule

\multicolumn{17}{c}{\textit{w Re-ranking}}   \\  \midrule
             Sparse Ret.                 &                   BM25                & Sentence                    & 26.3  & 37.5  & 56.7  & 65.6  & 31.5  & 37.1  & 39.3  & 43.1  & 35.6  & 43.4  & 58.5  & 64.2 & 41.3 & 48.5  \\ \midrule
\multirow{5}{*}{Dense Ret.}       & \multirow{2}{*}{ Contriever} & Passage                     & 26.5  & {37.7}  & 57.5  & {66.1}  & 26.2  & {37.2}  & 33.6  & {38}    & 35.4  & {43.7}  & 53.9  & {57.9} & 38.9 & 46.8  \\
                              &                                    & Sentence                    & 28.5  & {37.2}  & 60.9  & {67}    & 32.9  & {38.4}  & 38.3  & {42.7}  & 39    & {44}    & 60.7  & {63.4} & 43.4 & 48.8  \\ \cmidrule{2-17} 
                              & \multirow{2}{*}{ DPR}  & Passage                     & 36.5  & {42.1}  & 62.3  & {67.3}  & 25.3  & {35.4}  & 31.5  & {36}    & 38.9  & {44.6}  & 52.5  & {56.5} & 41.2 & 47.0  \\
                              &                                    & Sentence                    & 38.5  & {42.5}  & 64.3  & {68.2}  & 33.1  & {36}    & 35.8  & {40.4}  & 41.4  & {45.6}  & 59    & {62.7} & 45.4 & 49.2  \\ \midrule
\multirow{5}{*}{Supervised Rer.}   & \multirow{2}{*}{ MonoT5}     & Passage                     & 33.6  & {40.7}  & 62.1  & {67.6}  & 37.1  & {40}    & 37.8  & {41.5}  & 37.4  & {44.7}  & 58.7  & {62.3} & 44.5 & 49.5 \\
                              &                                    & Sentence                    & 37.4  & {42.3}  & 64.9  & {68.2}  & 39.5  & {39.5}  & 42.1  & {44.6}  & 41.4  & {44}    & 64.2  & {65.1} & 48.3 & 50.6  \\ \cmidrule{2-17} 
                              & \multirow{2}{*}{ RankT5}     & Passage                     & 35.4  & {41.4}  & 63.3  & {67.7}  & 39.2  & {40}    & 37.9  & {40.8}  & 37.8  & {44.5}  & 59.2  & {63.0} & 45.5 & 49.6    \\
                              &                                    & Sentence                    & 36.9  & {42.1}  & 64    & {67.9}  & 39.9  & {39.5}  & 42.8  & {43.9}  & 40.2  & {45.7}  & 65.6  & {66.5} & 48.2 & 50.9  \\ \midrule
\multirow{2}{*}{Unsupervised Rer.} & \multirow{2}{*}{ RG}         & Passage                     & 35.9  & {41.9}  & 65.7  & {68.8}  & 34    & {39.3}  & 27    & {30.1}  & 40.2  & {45}    & 60.9  & {63.5} & 44.0 & 48.1  \\
                              &                                    & Sentence                    & 39.2  & {42.9}  & 67.1  & {68.8}  & 37.2  & {39.8}  & 41.5  & {44.6}  & 42.1  & {47.3}  & 64.7  & {66.9} & \textbf{48.6} & \textbf{51.7}                                                                                                                                                                                                                                                                                                                        
% \\ \midrule
% \multicolumn{17}{c}{\textit{w/ Re-ranking}}  \\ \midrule
%              Sparse Ret.                &                   BM25                & Sentence  &    22.1  & {33.5}  & 50.1  & {62.0}    & 26.5  & {33.6}  & 39.3  & {43.1}  & 32.2  & {41.2}  & 51.5  & {60.4} & 37.0 & 45.6  \\ \midrule
% \multirow{5}{*}{Dense Ret.}       & \multirow{2}{*}{Contriever} & Passage                     & 26.0    & {37.2}  & 56.4  & {66.0}    & 23.7  & {35.3}  & 33.6  & {38.0}    & 36.3  & {44.6}  & 51.0    & {56} & 37.8 & 46.2 \\
%                               &                                    & Sentence                    & 28.0    & {37.6}  & 59.4  & {67.5}  & 32.5  & {39.0}    & 38.3  & {42.7}  & 40.5  & {45.4}  & 58.7  & {63.5} & 42.9 & 49.3   \\ \cmidrule{2-17} 
%                               & \multirow{2}{*}{DPR}  & Passage                     & 39.2  & {46.5}  & 61.8  & {68.8}  & 22.8  & {33.4}  & 31.5  & {36}    & 38.5  & {44.5}  & 48.0    & {53.6} & 40.3 & 47.1  \\
%                               &                                    & Sentence                    & 41.9  & {46.7}  & 65.3  & {69.8}  & 31.8  & {38.0}    & 35.8  & {40.4}  & 40.7  & {48.1}  & 57.0    & {62.1} & 45.4 & 50.9  \\ \midrule
% \multirow{5}{*}{Supervised Re-r.}   & \multirow{2}{*}{MonoT5}     & Passage                     & 35.4  & {43.9}  & 62.8  & {69.1}  & 38.3  & {42.3}  & 37.8  & {41.5}  & 39.3  & {46.8}  & 58.4  & {63.2} & 45.3 & 51.1 \\
%                               &                                    & Sentence                    & 40.5  & {46.3}  & 65.8  & {70.3}  & 41.9  & {41.8}  & 42.1  & {44.6}  & 42.2  & {48.6}  & 64.0    & {68.0} & 49.4 & 53.3   \\ \cmidrule{2-17} 
%                               & \multirow{2}{*}{RankT5}     & Passage                     & 38.0    & {44.7}  & 64.5  & {70.0}    & 41.5  & {43.5}  & 37.9  & {40.8}  & 39.0    & {46.5}  & 59.8  & {64.2} & 46.8 & 51.6  \\
%                               &                                    & Sentence                    & 39.7  & {46.0}    & 65.5  & {69.9}  & 42.4  & {41.8}  & 42.8  & {43.9}  & 39.0    & {48.5}  & 65.6  & {68.5} & 49.2 & 53.1  \\ \midrule
% \multirow{2}{*}{Unsupervised Re-r.} & \multirow{2}{*}{RG}         & Passage                     & 37.6  & {44.9}  & 66.3  & {71.0}    & 33.5  & {40.8}  & 27.0    & {30.1}  & 40.2  & {46.9}  & 60.8  & {63.4} & 44.2 & 49.5  \\
%                               &                                    & Sentence                    & 41.7  & {47.4}  & 68.5  & {71.7}  & 37.5  & {41.5}  & 41.5  & {44.6}  & 43.8  & {49.4}  & 65.4  & {68.8} & \textbf{49.7} & \textbf{53.9}  
\\ \bottomrule
\end{tabular}%
}
\begin{tablenotes}
\item[* RQA uses a specific GCS document from the dataset instead of the top-20, allowing for a variable number of top-\(N\) retrieved documents.] 
\end{tablenotes}
\vspace{-0.1in}
\end{threeparttable}
% \label{tab:main1_20}
\end{table*}

==> table/main2.tex <==
\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll | ccc | ccc | ccc | ccc}
\toprule 
\multirow{2}{*}{\textbf{Type}}    & \multirow{2}{*}{\textbf{Model}}             & \multirow{2}{*}{\textbf{Granularity}} & \multicolumn{3}{c|}{\textbf{MFQA}}            & \multicolumn{3}{c|}{\textbf{Qasper}}           & \multicolumn{3}{c|}{\textbf{NarrativeQA}}           &  \multicolumn{3}{c}{\textbf{AVG.}}            \\ 

                              &                                    &    & L=500 & L=1000 & L=2000 & L=500 & L=1000 & L=2000 & L=500 & L=1000 & L=2000 & L=500 & L=1000 & L=2000 \\ \midrule
% \multicolumn{15}{c}{\textit{w/o Retrieval}} \\ \midrule
% - & - & - & \multicolumn{3}{c|}{26.9} & \multicolumn{3}{c|}{15.9} & \multicolumn{3}{c|}{14.4} & \multicolumn{3}{c}{19.0} \\ \midrule 
\multicolumn{15}{c}{\textit{w/o Re-ranking}} \\ \midrule
- & - & - & 22.1 & 25.8 & 28.6 & 10.8 & 13.7 & 18.9 & 8.8 & 10.3 & 13.1 & 13.9 & 16.6 & 20.0 \\ \midrule 
\multicolumn{15}{c}{\textit{w/ Re-ranking}} \\ \midrule
 Sparse Ret. & BM25 & sentence & 27.3 & 28.6 & 29.8 & 20.0 & 16.3 & 19.5 & 10.8 & 11.5 & 13.9 & 19.4 & 18.8 & 21.1  \\ \midrule
 \multirow{5}{*}{Dense Ret.} & \multirow{2}{*}{Contriever} & passage & 27.3 & 26.3 & 29.5 & 21.8 & 19.1 & 18.7 & 11.0 & 12.0 & 12.9 & 20.0 & 19.1 & 20.4 \\ 
 & & sentence & 26.3 & 27.9 & 30.3 & 21.2 & 19.7 & 19.6 & 11.1 & 13.5 & 16.0 & 19.5 & 20.4 & 21.9 \\ \cmidrule{2-15}
  & \multirow{2}{*}{DPR} & passage & 26.5 & 26.6 & 29.5 & 16.5 & 16.6 & 17.7 & 11.5 & 13.5 & 12.7 & 18.2 & 18.9 & 19.9 \\ 
 & & sentence & 26.9 & 27.2 & 30.7 & 21.5 & 18.9 & 19.5 & 13.2 & 13.9 & 15.9 & 20.5 & 20.0 & 22.1 \\ \midrule
 \multirow{5}{*}{Supervised Rer.} & \multirow{2}{*}{MonoT5} & passage & 29.0 & 27.7 & 29.9 & 20.6 & 20.1 & 19.9 & 12.1 & 11.1 & 13.5 & 20.6 & 19.6 & 21.1 \\ 
 & & sentence & 28.9 & 29.3 & 30.2 & 23.1 & 18.6 & 21.7 & 12.0 & 15.0 & 16.7 & 21.3 & \textbf{21.0} & \textbf{22.9}\\ \cmidrule{2-15}
  & \multirow{2}{*}{RankT5} & passage & 29.3 & 29.5 & 30.0 & 22.2 & 18.8 & 20.5 & 10.6 & 11.4 & 11.3 & 20.7 & 19.9 & 20.6 \\ 
 & & sentence & 27.8 & 30.2 & 29.3 & 23.0 & 18.7 & 19.2 & 12.3 & 14.1 & 15.1 & 21.0 & \textbf{21.0} & 21.2\\ \midrule
\multirow{2}{*}{Unsupervised Rer.} & \multirow{2}{*}{RG} & passage & 28.0 & 28.4 & 29.1 & 24.1 & 19.1 & 19.5 & 12.6 & 13.8 & 12.2 & \textbf{21.6} & 20.4 & 20.3 \\ 
 & & sentence & 26.8 & 28.1 & 29.9 & 24.2 & 20.4 & 20.7 & 9.9 & 12.7 & 14.4 & 20.3 & 20.4 & 21.7 \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:main2}
\end{table*}

==> table/new_main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{lscape}

\begin{table*}[t!]
\caption{\small Comparative performance of sentence-level (\textit{DSLR}) and passage-level re-ranking methods across multiple open-domain QA datasets. Results are presented for two context lengths (\(L\)=100 and \(L\)=500), using sparse and dense retrievers, and both supervised and unsupervised re-rankers, for the top-100 retrieved documents. The best performances are in \textbf{bold}.}
\vspace{-0.1in}
\small
\centering

\begin{threeparttable}
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll | cc | cc | cc | cc | cc | cc | cc}
\toprule 
\multirow{2}{*}{\textbf{Type}}    & \multirow{2}{*}{\textbf{Re-ranker}}             & \multirow{2}{*}{\textbf{Granularity}} & \multicolumn{2}{c|}{\textbf{NQ}}            & \multicolumn{2}{c|}{\textbf{TQA}}           & \multicolumn{2}{c|}{\textbf{SQD}}           & \multicolumn{2}{c|}{\textbf{RQA}\tnote{*}}           & \multicolumn{2}{c|}{\textbf{SQ}} & \multicolumn{2}{c|}{\textbf{BASQ}} & \multicolumn{2}{c}{\textbf{AVG.}}            \\ 

                              &                                    &    & # tok& \textit{L}=500 & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 & \textit{L}=100 & \textit{L}=500 \\ \midrule
\multicolumn{17}{c}{\textit{w/o Re-ranking}}   \\  \midrule
- & - & -  & 25.5  & {34.9}  & 58    & {64.6}  & 28.5  & {35.9}  & 37    & {40.1}  & 33.9  & {40.9}  & 56.8  & {59.5} & 40.0 & 46.0 \\ \midrule
% \multicolumn{17}{c}{\textit{w/Re-ranking}}   \\  \midrule

% \multicolumn{17}{c}{\textit{Top-20 Documents Re-ranking}}   \\  \midrule
%              Sparse Ret.                 &                   BM25                & Sentence                    & 26.3  & 37.5  & 56.7  & 65.6  & 31.5  & 37.1  & 39.3  & 43.1  & 35.6  & 43.4  & 58.5  & 64.2 & 41.3 & 48.5  \\ \midrule
% \multirow{5}{*}{Dense Ret.}       & \multirow{2}{*}{ Contriever} & Passage                     & 26.5  & {37.7}  & 57.5  & {66.1}  & 26.2  & {37.2}  & 33.6  & {38}    & 35.4  & {43.7}  & 53.9  & {57.9} & 38.9 & 46.8  \\
%                               &                                    & Sentence                    & 28.5  & {37.2}  & 60.9  & {67}    & 32.9  & {38.4}  & 38.3  & {42.7}  & 39    & {44}    & 60.7  & {63.4} & 43.4 & 48.8  \\ \cmidrule{2-17} 
%                               & \multirow{2}{*}{ DPR}  & Passage                     & 36.5  & {42.1}  & 62.3  & {67.3}  & 25.3  & {35.4}  & 31.5  & {36}    & 38.9  & {44.6}  & 52.5  & {56.5} & 41.2 & 47.0  \\
%                               &                                    & Sentence                    & 38.5  & {42.5}  & 64.3  & {68.2}  & 33.1  & {36}    & 35.8  & {40.4}  & 41.4  & {45.6}  & 59    & {62.7} & 45.4 & 49.2  \\ \midrule
% \multirow{5}{*}{Supervised Rer.}   & \multirow{2}{*}{ MonoT5}     & Passage                     & 33.6  & {40.7}  & 62.1  & {67.6}  & 37.1  & {40}    & 37.8  & {41.5}  & 37.4  & {44.7}  & 58.7  & {62.3} & 44.5 & 49.5 \\
%                               &                                    & Sentence                    & 37.4  & {42.3}  & 64.9  & {68.2}  & 39.5  & {39.5}  & 42.1  & {44.6}  & 41.4  & {44}    & 64.2  & {65.1} & 48.3 & 50.6  \\ \cmidrule{2-17} 
%                               & \multirow{2}{*}{ RankT5}     & Passage                     & 35.4  & {41.4}  & 63.3  & {67.7}  & 39.2  & {40}    & 37.9  & {40.8}  & 37.8  & {44.5}  & 59.2  & {63.0} & 45.5 & 49.6    \\
%                               &                                    & Sentence                    & 36.9  & {42.1}  & 64    & {67.9}  & 39.9  & {39.5}  & 42.8  & {43.9}  & 40.2  & {45.7}  & 65.6  & {66.5} & 48.2 & 50.9  \\ \midrule
% \multirow{2}{*}{Unsupervised Rer.} & \multirow{2}{*}{ RG}         & Passage                     & 35.9  & {41.9}  & 65.7  & {68.8}  & 34    & {39.3}  & 27    & {30.1}  & 40.2  & {45}    & 60.9  & {63.5} & 44.0 & 48.1  \\
%                               &                                    & Sentence                    & 39.2  & {42.9}  & 67.1  & {68.8}  & 37.2  & {39.8}  & 41.5  & {44.6}  & 42.1  & {47.3}  & 64.7  & {66.9} & \textbf{48.6} & \textbf{51.7}                                                                                                                                                                                                                                                                                                                        
% \\ \midrule
\multicolumn{17}{c}{\textit{w Re-ranking}}  \\ \midrule
             Sparse Ret.                &                   BM25                & Sentence  &    22.1  & {33.5}  & 50.1  & {62.0}    & 26.5  & {33.6}  & 39.3  & {43.1}  & 32.2  & {41.2}  & 51.5  & {60.4} & 37.0 & 45.6  \\ \midrule
\multirow{5}{*}{Dense Ret.}       & \multirow{2}{*}{Contriever} & Passage                     & 26.0    & {37.2}  & 56.4  & {66.0}    & 23.7  & {35.3}  & 33.6  & {38.0}    & 36.3  & {44.6}  & 51.0    & {56} & 37.8 & 46.2 \\
                              &                                    & Sentence                    & 28.0    & {37.6}  & 59.4  & {67.5}  & 32.5  & {39.0}    & 38.3  & {42.7}  & 40.5  & {45.4}  & 58.7  & {63.5} & 42.9 & 49.3   \\ \cmidrule{2-17} 
                              & \multirow{2}{*}{DPR}  & Passage                     & 39.2  & {46.5}  & 61.8  & {68.8}  & 22.8  & {33.4}  & 31.5  & {36}    & 38.5  & {44.5}  & 48.0    & {53.6} & 40.3 & 47.1  \\
                              &                                    & Sentence                    & 41.9  & {46.7}  & 65.3  & {69.8}  & 31.8  & {38.0}    & 35.8  & {40.4}  & 40.7  & {48.1}  & 57.0    & {62.1} & 45.4 & 50.9  \\ \midrule
\multirow{5}{*}{Supervised Re-r.}   & \multirow{2}{*}{MonoT5}     & Passage                     & 35.4  & {43.9}  & 62.8  & {69.1}  & 38.3  & {42.3}  & 37.8  & {41.5}  & 39.3  & {46.8}  & 58.4  & {63.2} & 45.3 & 51.1 \\
                              &                                    & Sentence                    & 40.5  & {46.3}  & 65.8  & {70.3}  & 41.9  & {41.8}  & 42.1  & {44.6}  & 42.2  & {48.6}  & 64.0    & {68.0} & 49.4 & 53.3   \\ \cmidrule{2-17} 
                              & \multirow{2}{*}{RankT5}     & Passage                     & 38.0    & {44.7}  & 64.5  & {70.0}    & 41.5  & {43.5}  & 37.9  & {40.8}  & 39.0    & {46.5}  & 59.8  & {64.2} & 46.8 & 51.6  \\
                              &                                    & Sentence                    & 39.7  & {46.0}    & 65.5  & {69.9}  & 42.4  & {41.8}  & 42.8  & {43.9}  & 39.0    & {48.5}  & 65.6  & {68.5} & 49.2 & 53.1  \\ \midrule
\multirow{2}{*}{Unsupervised Re-r.} & \multirow{2}{*}{RG}         & Passage                     & 37.6  & {44.9}  & 66.3  & {71.0}    & 33.5  & {40.8}  & 27.0    & {30.1}  & 40.2  & {46.9}  & 60.8  & {63.4} & 44.2 & 49.5  \\
                              &                                    & Sentence                    & 41.7  & {47.4}  & 68.5  & {71.7}  & 37.5  & {41.5}  & 41.5  & {44.6}  & 43.8  & {49.4}  & 65.4  & {68.8} & \textbf{49.7} & \textbf{53.9}  \\ \bottomrule
\end{tabular}%
}
\begin{tablenotes}
\item[* RQA uses a specific GCS document from the dataset instead of the top-100, allowing for a variable number of top-\(N\) retrieved documents.] 
\end{tablenotes}
\vspace{-0.125in}
\end{threeparttable}
\label{tab:main1}
\end{table*}

==> table/sentence-level-reranking_is_good.tex <==

% \begin{table}
%     \centering
%     \begin{tabular}{ccc}
%          &  Passage& Sentence\\
%          BM25&  25.5& 22.1\\
%          Contriever&  26.0& 28.0\\
%          DPR&  39.2& 41.9\\
%          MonoT5&  35.4& 40.5\\
%          RankT5&  38.0& 39.7\\
%          RG&  37.6& 41.7\\
%     \end{tabular}
%     \caption{Comparative performance of sentence-level versus passage-level re-ranking on the NQ dataset with a context length of 100 words. Best performances are highlighted in \textbf{bold}}
%     \label{tab:sentence-reranking}
% \end{table}

\begin{table}
    \small
    \centering
    \begin{tabular}{ccc}
        \toprule
        & \textbf{Passage} & \textbf{Sentence} \\
        \midrule
        BM25 & 25.5 & 22.1 \\
        Contriever & 26.0 & 28.0 \\
        DPR & 39.2 & \textbf{41.9} \\
        MonoT5 & 35.4 & 40.5 \\
        RankT5 & 38.0 & 39.7 \\
        RG & 37.6 & 41.7 \\
        \bottomrule
    \end{tabular}
    \caption{Comparative performance of sentence-level and passage-level re-ranking on the NQ with a context length of 100 words. The best performance is highlighted in \textbf{bold}.}
    \label{tab:sentence-reranking}
\end{table}
